Periodic Activation Functions Induce Stationarity

Neural network models are known to reinforce hidden data biases, making them unreliable and difficult to interpret. We seek to build models that `know what they do not know' by introducing inductive biases in the function space. We show that periodic activation functions in Bayesian neural networks establish a connection between the prior on the network weights and translation-invariant, stationary Gaussian process priors. Furthermore, we show that this link goes beyond sinusoidal (Fourier) activations by also covering triangular wave and periodic ReLU activation functions. In a series of experiments, we show that periodic activation functions obtain comparable performance for in-domain data and capture sensitivity to perturbed inputs in deep neural networks for out-of-domain detection.

==> tbl/KFACshort-nlpd-acc.tex <==


%NLPD_ACC (this table has been automatically generated, do not alter manually)
                          &       \multicolumn{2}{c}{\sc diabetes}        &         \multicolumn{2}{c}{\sc adult}         &       \multicolumn{2}{c}{\sc connect-4}       &        \multicolumn{2}{c}{\sc covtype}        \\
($n$, $d$)                &         \multicolumn{2}{c}{(768, 8)}          &        \multicolumn{2}{c}{(45222, 14)}        &        \multicolumn{2}{c}{(67556, 42)}        &       \multicolumn{2}{c}{(581912, 54)}        \\
($c$, $n_\textrm{batch}$) &          \multicolumn{2}{c}{(2, 50)}          &         \multicolumn{2}{c}{(2, 500)}          &         \multicolumn{2}{c}{(3, 500)}          &         \multicolumn{2}{c}{(7, 500)}          \\
\midrule
                          &         NLPD          &          ACC          &         NLPD          &          ACC          &         NLPD          &          ACC          &         NLPD          &          ACC          \\
\midrule
ReLU                      &    $0.47{\pm}0.04$    &    $0.77{\pm}0.04$    &    $0.31{\pm}0.01$    &  $\bf 0.85{\pm}0.00$  &    $0.52{\pm}0.01$    &    $0.82{\pm}0.00$    &    $0.18{\pm}0.00$    &    $0.93{\pm}0.00$    \\
loc RBF                   &  $\bf 0.47{\pm}0.04$  &    $0.76{\pm}0.04$    &    $0.31{\pm}0.01$    &    $0.85{\pm}0.00$    &  $\bf 0.50{\pm}0.01$  &    $0.82{\pm}0.00$    &    $0.18{\pm}0.00$    &    $0.93{\pm}0.00$    \\
glob RBF (sin)            &    $0.48{\pm}0.05$    &  $\bf 0.78{\pm}0.04$  &    $0.31{\pm}0.01$    &    $0.85{\pm}0.00$    &    $0.54{\pm}0.02$    &    $0.82{\pm}0.00$    &    $0.17{\pm}0.00$    &    $0.93{\pm}0.00$    \\
glob RBF (tri)            &    $0.48{\pm}0.05$    &    $0.77{\pm}0.05$    &    $0.31{\pm}0.01$    &    $0.85{\pm}0.00$    &    $0.54{\pm}0.02$    &  $\bf 0.82{\pm}0.00$  &    $0.17{\pm}0.00$    &    $0.93{\pm}0.00$    \\
glob RBF (sincos)         &    $0.48{\pm}0.05$    &    $0.76{\pm}0.04$    &    $0.31{\pm}0.00$    &    $0.85{\pm}0.00$    &    $0.54{\pm}0.01$    &    $0.82{\pm}0.00$    &    $0.17{\pm}0.00$    &    $0.93{\pm}0.00$    \\
glob RBF (prelu)          &    $0.48{\pm}0.05$    &    $0.77{\pm}0.04$    &  $\bf 0.31{\pm}0.01$  &    $0.85{\pm}0.00$    &    $0.54{\pm}0.02$    &    $0.82{\pm}0.00$    &  $\bf 0.17{\pm}0.00$  &  $\bf 0.93{\pm}0.00$  \\


==> tbl/short-nlpd-acc.tex <==


%NLPD_ACC (this table has been automatically generated, do not alter manually)
                          &       \multicolumn{2}{c}{\sc diabetes}        &         \multicolumn{2}{c}{\sc adult}         &       \multicolumn{2}{c}{\sc connect-4}       &        \multicolumn{2}{c}{\sc covtype}        \\
($n$, $d$)                &         \multicolumn{2}{c}{(768, 8)}          &        \multicolumn{2}{c}{(45222, 14)}        &        \multicolumn{2}{c}{(67556, 42)}        &       \multicolumn{2}{c}{(581912, 54)}        \\
($c$, $n_\textrm{batch}$) &          \multicolumn{2}{c}{(2, 50)}          &         \multicolumn{2}{c}{(2, 500)}          &         \multicolumn{2}{c}{(3, 500)}          &         \multicolumn{2}{c}{(7, 500)}          \\
\midrule
                          &         NLPD          &          ACC          &         NLPD          &          ACC          &         NLPD          &          ACC          &         NLPD          &          ACC          \\
\midrule
ReLU                      &    $0.53{\pm}0.07$    &    $0.75{\pm}0.03$    &    $0.38{\pm}0.15$    &    $0.79{\pm}0.18$    &    $0.54{\pm}0.12$    &    $0.79{\pm}0.04$    &    $0.19{\pm}0.00$    &    $0.92{\pm}0.00$    \\
loc RBF                   &    $0.49{\pm}0.05$    &    $0.76{\pm}0.04$    &  $\bf 0.33{\pm}0.01$  &    $0.85{\pm}0.00$    &  $\bf 0.47{\pm}0.01$  &  $\bf 0.81{\pm}0.00$  &    $0.19{\pm}0.00$    &    $0.93{\pm}0.00$    \\
glob RBF (sin)            &    $0.51{\pm}0.05$    &    $0.76{\pm}0.04$    &    $0.35{\pm}0.03$    &    $0.85{\pm}0.00$    &    $0.51{\pm}0.05$    &    $0.81{\pm}0.01$    &  $\bf 0.18{\pm}0.00$  &  $\bf 0.93{\pm}0.00$  \\
glob RBF (tri)            &    $0.53{\pm}0.07$    &    $0.73{\pm}0.04$    &    $0.33{\pm}0.01$    &    $0.85{\pm}0.00$    &    $0.51{\pm}0.05$    &    $0.81{\pm}0.01$    &    $0.19{\pm}0.01$    &    $0.92{\pm}0.00$    \\
glob RBF (sincos)         &                      ---                      &    $0.37{\pm}0.10$    &    $0.83{\pm}0.07$    &    $0.54{\pm}0.07$    &    $0.80{\pm}0.01$    &    $0.18{\pm}0.01$    &    $0.93{\pm}0.00$    \\
glob RBF (prelu)          &    $0.52{\pm}0.06$    &    $0.76{\pm}0.04$    &    $0.34{\pm}0.01$    &  $\bf 0.85{\pm}0.00$  &    $0.50{\pm}0.01$    &    $0.81{\pm}0.00$    &    $0.19{\pm}0.01$    &    $0.92{\pm}0.00$    \\

